Message Passing-Based 9-D Cooperative Localization and Navigation with Embedded Particle Flow

Cooperative localization (CL) is an important technology for innovative services such as location-aware communication networks, modern convenience, and public safety. We consider wireless networks with mobile agents that aim to localize themselves by performing pairwise measurements amongst agents and exchanging their location information. Belief propagation (BP) is a state-of-the-art Bayesian method for CL. In CL, particle-based implementations of BP often are employed that can cope with non-linear measurement models and state dynamics. However, particle-based BP algorithms are known to suffer from particle degeneracy in large and dense networks of mobile agents with high-dimensional states. This paper derives the messages of BP for CL by means of particle flow, leading to the development of a distributed particle-based message-passing algorithm which avoids particle degeneracy. Our combined particle flow-based BP approach allows the calculation of highly accurate proposal distributions for agent states with a minimal number of particles. It outperforms conventional particle-based BP algorithms in terms of accuracy and runtime. Furthermore, we compare the proposed method to a centralized particle flow-based implementation, known as the exact Daum-Huang filter, and to sigma point BP in terms of position accuracy, runtime, and memory requirement versus the network size. We further contrast all methods to the theoretical performance limit provided by the posterior Cram\'er-Rao lower bound (PCRLB). Based on three different scenarios, we demonstrate the superiority of the proposed method.

==> input_files/inference_model.tex <==

\begin{figure*}[t]
\subfloat[FG representation for joint cooperative localization and model parameter estimation \newline where all model parameters are captured in one node]{\hspace{-2cm}
{\input{figures/FG_mirrow.tex}\label{fig:FG_mirrow}}}
\subfloat[This FG is an example how node $\alpha$ can be further factorized]{\hspace{-1.5cm}
{\input{figures/FG_alpha_small.tex}\label{fig:FG_alpha}}}\hfill
\caption{This figure shows a FG for joint cooperative localization and model parameter estimation. Factors in purple are involved in updates of the agent states whereas factors in yellow are involved in updates of the parameter state. Factors in blue correspond to prior knowledge and information from anchors.}
\label{fig:FG}
\end{figure*}


\section{Inference model}
\label{sec:infM}
This section describes the inference model to estimate position and orientation of the agents based on their marginal PDFs, as well as model parameters and the measurement noise. We define the model parameter vector as ${\boldsymbol{\alpha} = [P,n,\boldsymbol{\xi}^\text{T},\sigma]^\text{T}}$ that consists of the reference path-loss $P$ at distance $d_0$, the path-loss exponent $n$, the model parameters of the antenna pattern $\boldsymbol{\xi}$ and the shadowing standard deviation $\sigma$. We use a fully continuous representation for the unknown parameters. Since the measurements between nodes are independent of each other, the posterior PDF in \eqref{eq:contJointPost} can be factorized as
\begin{align}
f(\boldsymbol{\theta},\boldsymbol{\alpha}|\mathbf{z}) &\propto f(\boldsymbol{\alpha}) \prod_{i \in \mathcal{C}} f(\boldsymbol{\theta}_i) \prod_{a \in \mathcal{A}} f(\bar{z}_{i,a}|\boldsymbol{\theta}_{i},\boldsymbol{\theta}_{a},\boldsymbol{\alpha})  \nonumber \\
& \times  \prod_{j \in \mathcal{D}_i}  f(\underline{z}_{i,j}|\boldsymbol{\theta}_{i},\boldsymbol{\theta}_{j},\boldsymbol{\alpha})
\label{eq:joint_post}
\end{align} which consists of the prior PDF of the model parameters $f(\boldsymbol{\alpha})$, the prior PDF $f(\boldsymbol{\theta}_i)$ of agent state $i$, the likelihood function $f(\bar{z}_{a,i}|\boldsymbol{\theta}_{i},\boldsymbol{\theta}_{a},\boldsymbol{\alpha})$ which is a function of $i$th agent state, the model parameters and parametrized by the $a$th anchor state (which is known) and the likelihood function $f(\underline{z}_{i,j}|\boldsymbol{\theta}_{i},\boldsymbol{\theta}_{j},\boldsymbol{\alpha})$ which is a function of the $i$th agent state, the $j$th agent state with $i\neq j$ and the model parameters $\boldsymbol{\alpha}$.

Since we perform estimation based on the marginal posterior PDF of each agent state, we define the \textit{not-integrate} notation as mentioned in \cite{KschischangTIT2001}. Instead of indicating which variables are marginalized out, we define the ones over which we do not integrate. For example if $h(\cdot)$ is a function that depends on the continuous variables $\boldsymbol{\theta}_1$, $\boldsymbol{\theta}_2$ and $\boldsymbol{\theta}_3$, the \textit{not-integrate} for $\boldsymbol{\theta}_3$ is defined as
\begin{align}
\int h(\boldsymbol{\theta}_1,\boldsymbol{\theta}_2,\boldsymbol{\theta}_3) d\boldsymbol{\theta}_{\sim 3} & \coloneqq \iint h(\boldsymbol{\theta}_1,\boldsymbol{\theta}_2,\boldsymbol{\theta}_3) d\boldsymbol{\theta}_1 d\boldsymbol{\theta}_2 \label{eq:notInt}
\end{align}

With the help of the \textit{not-integrate} notation in \eqref{eq:notInt}, the marginal posterior PDFs of state $\boldsymbol{\theta}_i$  and $\boldsymbol{\alpha}$ are given by
\begin{align}
f(\boldsymbol{\theta}_i|\mathbf{z}) &= \iint f(\boldsymbol{\theta},\boldsymbol{\alpha}|\mathbf{z}) d\boldsymbol{\alpha} d\boldsymbol{\theta}_{\sim i} \label{eq:marg_post_agent}\\
%
f(\boldsymbol{\alpha}|\mathbf{z}) &= \int f(\boldsymbol{\theta},\boldsymbol{\alpha}|\mathbf{z}) d\boldsymbol{\theta}
\label{eq:marg_post_alpha}
\end{align}
where $\int d\boldsymbol{\theta}_{\sim i}$ denotes the marginalization of all states $\boldsymbol{\theta}$ except $\boldsymbol{\theta}_{i}$.


\subsection{Likelihood} 
For a Gaussian noise model given in \eqref{eq:measModelAP}, the likelihood function for a measurement in-between two nodes can be written in the form of
\begin{equation}
f(z_{i,j}|\boldsymbol{\theta}_{i},\boldsymbol{\theta}_{j},\boldsymbol{\alpha}) = \frac{1}{\sqrt{2\pi \sigma^2}} \text{exp}\left(\frac{1}{2\sigma^2} (z_{i,j} - \tilde{z}_{i,j})^2  \right)
\label{eq:lhf}
\end{equation}
with
\begin{equation}
\tilde{z}_{i,j} = L(P,n,d_{i,j}) + \Psi(\boldsymbol{\xi},{\phi}_{i,j} ,{\phi}_{j,i})
\label{eq:lhf_param}
\end{equation}
and $\boldsymbol{\theta}_i = [\mathbf{x}_i \iist\varphi_i]^\text{T} $.

==> input_files/synthResults.tex <==
%
%\begin{figure*}[t]
%\centering
%\subfloat[$\sigma$ = 0.1 m, $r_\text{max}$ = 20 m]
%{\input{figures/convergence_Annealing_rmax20_sigma_0p1_agents_100.tex}\label{fig:flowConvergence_a}}
%\subfloat[$\sigma$ = 1 m, $r_\text{max}$ = 20 m]{\hspace{-2mm}
%{\input{figures/convergence_Annealing_rmax20_sigma_1_agents_100.tex}\label{fig:flowConvergence_b}}}
%\subfloat[$\sigma$ = 3 m, $r_\text{max}$ = 20 m]{\hspace{-2mm}
%{\input{figures/convergence_Annealing_rmax20_sigma_3_agents_100.tex}\label{fig:flowConvergence_c}}} \\
%\subfloat[$\sigma$ = 0.1 m, $r_\text{max}$ = 25 m]
%{\input{figures/convergence_Annealing_rmax25_sigma_0p1_agents_100.tex}\label{fig:flowConvergence_d}}
%\subfloat[$\sigma$ = 1 m, $r_\text{max}$ = 25 m]{\hspace{-2mm}
%{\input{figures/convergence_Annealing_rmax25_sigma_1_agents_100.tex}\label{fig:flowConvergence_e}}}
%\subfloat[$\sigma$ = 3 m, $r_\text{max}$ = 25 m]{\hspace{-2mm}
%{\input{figures/convergence_Annealing_rmax25_sigma_3_agents_100.tex}\label{fig:flowConvergence_f}}} \hfill
%\pgfplotslegendfromname{EDH_BP_covReg}
%\caption{This figure shows the RMSE in m and the standard deviation of the MMSE for different values of $\alpha$. It is evaluated for two different interaction radii and three values of measurement noise with 200 particles. Each point is averaged over 100 simulation runs for a scenario with 100 randomly placed agents and 16 equally spaced anchors. The flow time $\lambda$ has 25 exponentially spaced values}
%\label{fig:flowConvergence}
%\end{figure*}


\begin{figure*}[t]
\centering
\subfloat[$\sigma$ = 0.1 m, $r_\text{max}$ = 20 m]
{\input{figures/final_static_RMSEvsAGENTS_rmax20_sigma_0p1.tex}\label{fig:algoVSagents_a}}
\subfloat[$\sigma$ = 1 m, $r_\text{max}$ = 20 m]{\hspace{-2mm}
{\input{figures/final_static_RMSEvsAGENTS_rmax20_sigma_1.tex}\label{fig:algoVSagents_b}}}
\subfloat[$\sigma$ = 3 m, $r_\text{max}$ = 20 m]{\hspace{-2mm}
{\input{figures/final_static_RMSEvsAGENTS_rmax20_sigma_3.tex}\label{fig:algoVSagents_c}}} \\
\subfloat[$\sigma$ = 0.1 m, $r_\text{max}$ = 25 m]
{\input{figures/final_static_RMSEvsAGENTS_rmax25_sigma_0p1.tex}\label{fig:algoVSagents_d}}
\subfloat[$\sigma$ = 1 m, $r_\text{max}$ = 25 m]{\hspace{-2mm}
{\input{figures/final_static_RMSEvsAGENTS_rmax25_sigma_1.tex}\label{fig:algoVSagents_e}}}
\subfloat[$\sigma$ = 3 m, $r_\text{max}$ = 25 m]{\hspace{-2mm}
{\input{figures/final_static_RMSEvsAGENTS_rmax25_sigma_3.tex}\label{fig:algoVSagents_f}}} \hfill
\pgfplotslegendfromname{finalStatic_RMSEvsAGENTS}
\caption{This figure shows the RMSE in m and the standard deviation of the MMSE for various numbers of agents. It is evaluated for two different interaction radii and three values of measurement noise. Each point is averaged over 100 simulation runs.}
\label{fig:algoVSagents}
\end{figure*}


\section{Evaluation of Algorithms}
\label{sec:Results}
In this section, we evaluate the algorithms based on static and dynamic networks for various network sizes and connectivities. We compare the performance in terms of the root-mean-square error (RMSE), the cumulative frequency (CF) and the execution time.

\subsection{Static Scenario}

In this section, we study the performance of the proposed method based on simulation in a static 2D scenario for different measurement uncertainties and network sizes. In addition, we compare it to state of the art particle based message passing algorithms described in Section~\ref{sec:BP}, indicated as SIR-BP, the Nonlienar-Least-Squares (NLLS) algorithm and the joint flow corresponding to the EDH where we resample according to \eqref{eq:jointWeights} and also \eqref{eq:margWeights}. For the BP algorithms we use $\sigma_k = 0.01$~m. The different uncertainties of the measurement model are given as $\V{\sigma} = [0.1,1,3]$~m. In the following simulations, we use 16 anchors and various numbers of agents defined as $N_\text{agent} = [50,100,150,200]$. The true agent positions are uniformly drawn for each realization on an area of 100~m$\times$100~m. The anchors are placed equally spaced on the support area. The prior distribution of the agent $i$s position is initialized with a Gaussian distribution where the mean value corresponds to the center of gravity of the anchors that have a connection to agent $i$ and a standard deviation of 29~m. This is equivalent to the standard deviation of a uniform distribution represented by the support area. The initial values of the NLLS are equivalent to the mean values of the prior distributions. For PF-BP, we use 25 exponentially spaced $\lambda$ steps. The communication of anchors and agents and agents and agents is restricted to a communication range $r_{\text{max}}$, which can have the values of 20~m and 25~m to simulate lower and higher connectivity. The scenario is similar to the one described in Section~\ref{sec:dyn}. A graphical representation is given there.



\subsubsection{Convergence Analysis of Flow}
We observe that for PF-BP, the convergence behavior regarding BP iterations is sometimes very poor. We can explain this effect due to a bias that occurs in the first iteration. After calculating the weights at the end of the flow, the covariance matrix of the biased agents can be extremely underestimated, which leads in the next BP iteration to a wrong consideration of the agents uncertainty. In the extreme case, the cooperating agents are treated in the same manner as anchors but with wrong positions which could lead to diverging agent states as indicated in Figure~\ref{fig:flowConvergence_a}. This is more frequent in scenarios with a low connectivity. Hence we analyzed the scenario with 100 agents and use 150 BP iterations to better capture this effect. We can tackle this problem by artificially enlarging the covariance matrix of the cooperative partners in the flow equation. It can be seen in Figure~\ref{fig:flowConvergence} how the speed of convergence increases if we use this heuristic but we can also see that if the additive covariance is too large, the achieved accuracy of the algorithm is not optimal. This is especially the case if the connectivity is high as indicated in Figure~\ref{fig:flowConvergence_d}-\ref{fig:flowConvergence_f}. To combine the better accuracy of the correct flow with the higher robustness and faster convergence of the heuristic, we decrease the additive covariance exponentially with the BP iterations. This is equivalent to an annealing strategy. The covariance matrix in \eqref{eq:A_i} and \eqref{eq:b_i} changes to
\begin{equation}
\V{P}_i = \text{diag}(\V{P}_i^{(0)},\V{P}_{\V{\chi}_{\Set{D}_i(1)}}^{(u-1)}+\V{1\!\!1} \alpha(u),\dots,\V{P}_{\V{\chi}_{\Set{D}_i(|\Set{D}_i|)}}^{(u-1)}+\V{1\!\!1} \alpha(u))
\end{equation}
with $\V{\alpha}$ being a vector of the length $U$ with exponentially decreasing steps between some maximum value and zero. Due to the static scenario, we drop the time index $k$. Since the additive value in the last BP iteration is equal to zero, the positioning performance does not suffer as we see in the following section where we are able to reach the PCRLB. \\


\subsubsection{Various numbers of agents}
\label{sec:varAgents}

In this section we evaluate the achievable accuracy of the algorithms for the scenarios defined in Section~\ref{sec:Results}. We compare our proposed method with a state of the art particle based BP algorithm with 2000 and 50000 particles, indicated as SIR-BP, a NLLS algorithm the performs a joint estimation of the position, the joint implementation of the PF according to Section~\ref{subsec:EDH} and the theoretical performance limit based on the PCRLB. For the PF-based methods, we use 200 particles. For the NLLS algorithm, we use the function \texttt{lsqnonlin} in MATLAB with the setting \texttt{levenberg-marquardt}. The results for different parameter settings and various numbers of agents are given in Figure~\ref{fig:algoVSagents}. For scenarios with lower interaction radius, SIR-BP hast the best performance in terms of accuracy. That is due to the fact that the network is not always fully localizable and SIR-BP can capture the multimodality. On the other hand, the computational complexity is quiet large since we use 50000 particles to achieve that accuracy. Therefor PF-BP results in a good trade-off between computational complexity like memory and runtime and accuracy. That is especially the case for the measurement model with $\sigma = 0.1$~m. The benefit in terms of runtime is shown in Section~\ref{sec:complexity}. NNLS and EDH perform always worse compared to the BP algorithms. The PF based methods as well as the NNLS use a gradient which could get stuck in a local minimum if the scenario is not fully localizable. That describes the discrepancy between SIR-BP and the other approaches. 

\begin{table}[t]
  \caption{Mean localizability  of scenarios in \%}
\begin{center}
  \begin{tabular}{| c | r | r | } \hline
$N_\text{agent}$ &  $r_{\text{max}} = 20$~m & $r_{\text{max}} = 25$~m   \\ \hline
50	 & 89.82 & 98.68   \\ \hline
100	 & 99.43 & 99.97  \\ \hline
150	 & 99.95 & 100.00   \\ \hline
200	 & 100.00 & 100.00  \\ \hline
 \end{tabular}
\end{center}
\label{tb:localizability}
\end{table}

\begin{figure}[t]
\centering
\subfloat[$r_\text{max}$ = 20 m]
{\input{figures/finalStatic_CDF_100runs_200agents_rmax20_sig0p1.tex}\label{fig:CDF_a}}\\
\subfloat[$r_\text{max}$ = 25 m]
{\input{figures/finalStatic_CDF_100runs_200agents_rmax25_sig0p1.tex}\label{fig:CDF_b}}\\
%\subfloat[convergence $r_\text{max}$ = 25 m]
%{\input{figures/convergence_Annealing_rmax25_sigma_0.1_agents_200.tex}\label{fig:CDF_conv}}\\
\pgfplotslegendfromname{CDF_0p1_200agents}
\caption{This figure shows the cumulative frequency of the positioning error for 200 agents and $\sigma = 0.1$~m for different algorithms and interaction radii as well as the convergence of the different algorithms.}
\label{fig:CDF}
\end{figure}


For scenarios with higher connectivity and a small measurement uncertainty, PF-BP has the best overall performance but for 200 agents the NLLS has a slightly higher accuracy. At a certain connectivity, the RMSE of SIR-BP reaches a plateau since more particles are needed to capture the information gain. This is clearly depicted in Figure~\ref{fig:algoVSagents_d}. We see that 2000 particles are too few for SIR-BP to even come close to the performance of the other algorithms. For 50000 particles, the plateau starts at 150 agents. That is not the case PF-BP and NLLS. We can also see that we are able to reach the PCRLB is the network is localizable. For larger uncertainty of the measurements, SIR-BP reaches the PCRLB even for 50 and 100 agents. PF-BP and NLLS have a similar performance in terms of accuracy and are also able to reach the PCRLB. 

If the connectivity is increased by increasing the number of agents, the PF-BP converges to the results of SIR-BP but still having the benefit of a lower computation time (see Section~\ref{sec:complexity}) and less used resources since we only used 200 particles for PF-BP. We can also argue that in a distributed estimation of the agent states, the communication overhead is much smaller for PF-BP since agents have to transmit only mean and covariance instead of the full particle based representation of the state as for SIR-BP. To determine the localizable agents, we use the algorithm proposed in \cite{ping2021MaxFlow}. The mean number of localizable agents for all simulation runs and scenarios is given in Table~\ref{tb:localizability}. If the scenario is localizable, we see that both message passing methods and the NLLS could reach the PCRLB whereas the joint EDH does not reach this lower bound. For the joint EDH there is still the problem of particle collapse since we resample the joint state with a small amount of particles. For large measurement uncertainty, the achievable accuracy is in the same magnitude as of the error due to calculating the MMSE of multimodal distributions. Therefore BP reaches the lower bound even though the scenario is not fully localizable.


We further analyse the accuracy of the positioning performance or the scenario with 200 agents and $\sigma = 0.1$~m. For that case, we show the cumulative frequency (CF) of the positioning error for different parameter settings of the algorithms in Figure~\ref{fig:CDF}. For the scenario with less connectivity, the proposed PF-BP method has a better performance in terms of accuracy but more outliers compared to the SIR-BP. Therefor the overall RMSE is a bit higher for the proposed method. Increasing the interaction radius by 5~m has a significant impact on performance of the investigated algorithms. The achievable accuracy of PF-BP is similar to the NLLS algorithm. In addition, we show how the accuracy of SIR-SBP increases with increasing number of particles. Comparing it to PF-BP, we see that we would need much more particles to reach the same achievable accuracy. Furthermore, we show the CF of the joint EDH with two different resampling strategies according to  \eqref{eq:jointWeights} and \eqref{eq:margWeights} which cannot reach the accuracy of the proposed method. This would only be the case if we have a fully connected network as in \cite{}. We also compared to Sigma-Point BP but for static scenarios the results are much worse compared to the other methods. This is due to the fact that SPBP converges only over time and is always biased if the mean of the prior distribution is not in the vicinity of the true position. The benefit of SPBP is displayed in the following section.





\begin{figure}[t]
\centering
\subfloat[$r_\text{max}$ = 20 m]
{\input{figures/TIMEvsAGENTS_rmax20_iteration_20_30.tex}}
\subfloat[$r_\text{max}$ = 25 m]
{\input{figures/TIMEvsAGENTS_rmax25_iteration_20_30.tex}}\\
\pgfplotslegendfromname{timeVSagents}
\caption{This figure shows the mean calculation time per run. It is evaluated for different interaction radii and averaged over all three measurement uncertainties and 100 simulation runs.}
\label{fig:timeVSagents}
\end{figure}




\subsubsection{Complexity}
\label{sec:complexity}
In this section we evaluate the complexity of the algorithms in terms of runtime for 20 BP iterations. Our results indicate that there is no significant change in the RMSE when using more iterations. We can see in Figure~\ref{fig:timeVSagents} how the computation time increases with increasing number of agents. This analysis shows, that the PF-BP is also faster or equivalent for the same or a better positioning accuracy than the comparison algorithms. The runtime of NLLS is of course independent of the BP iterations but it needs more time to converge if less information is available. If the uncertainty of the measurement model is higher, less particles are needed for SIR-BP which could decrease the runtime significantly. Using less particles for PF-BP would not lead to a significant decrease of runtime since at that level, the matrix inversion and multiplication is the limiting factor. For the investigated scenarios, the joint EDH has the best performance in terms of runtime, which could be insufficient if the positioning accuracy is poor as shown in Section~\ref{sec:varAgents}. We can conclude that for the model with the lowest uncertainty PF-BP is the best choice in terms of runtime and accuracy. For models with higher uncertainty or less connectivity, SIR-BP could be a better choice since the number of particles can be reduced significantly, leading to much shorter computation time.










